Optimized Asynchronous Passive Multi-Channel Discovery of Beacon-Enabled Networks

Neighbor discovery is a fundamental task for wireless networks deployment. It is essential for setup and maintenance of networks and is typically a precondition for further communication. In this work we focus on passive discovery of networks operating in multi-channel environments, performed by listening for periodically transmitted beaconing messages. It is well-known that performance of such discovery approaches strongly depends on the structure of the adopted Beacon Interval (BI) set, that is, set of intervals between individual beaconing messages. However, although imposing constraints on this set has the potential to make the discovery process more efficient, there is demand for high-performance discovery strategies for BI sets that are as general as possible. They would allow to cover a broad range of wireless technologies and deployment scenarios, and enable network operators to select BI's that are best suited for the targeted application and/or device characteristics. In the present work, we introduce a family of novel low-complexity discovery algorithms that minimize both the Expected Mean Discovery Time (EMDT) and the makespan, for a quite general family of BI sets. Notably, this family of BI sets completely includes BI's supported by IEEE 802.15.4 and a large part of BI's supported by IEEE 802.11. Furthermore, we present another novel discovery algorithm, based on an Integer Linear Program (ILP), that minimizes EMDT for arbitrary BI sets. In addition to analytically proving optimality, we numerically evaluate the proposed algorithms using different families of BI sets and compare their performance with the passive scan of IEEE 802.15.4 w.r.t. various performance metrics, such as makespan, EMDT, energy usage, etc.

==> GENALG.tex <==

\begin{comment}

\subsection{Sequence of Discovering Beacon Intervals}
\label{subsubsec:sequence_BI}

 

Figure~\ref{fig:intervalSequence} depicts listening schedules of STEPOPT and of GENOPT; a strategy that we will explain in detail in the next section. The beacon interval set is $B = \{1,2,3\}$ and the number of channels $|C| = 3$. We can see that the STEPOPT listening schedule first discovers all neighbors operating with $b_1$ on the three channels, then completes the scan for $b_2$ in time slot $t_5$. However, the scans of time slots $t_3$ on $c_0$, $t_4$ on $c_2$ and $t_5$ on $c_1$ will not result in any new discoveries for $b_3$ since on all three channels the time slot $t_{x-3}$ has already been scanned. Therefore, there are in total four time slots allocated for scanning on each channel even though $b_{max} = 3$.
The listening schedule of GENOPT completes the discovery of neighbors operating with $b_2$ on $c_1$ first, before neighbors using $b_1$ are discovered on $c_2$. This shift results in the minimum number of three time slots per channel to discover every neighbor operating with any $b \in B$. 

In Table~\ref{tab:intervalSequence} we show analytical results of the average discovery time for each beacon interval and for the complete beacon interval set. GENOPT achieves lower average discovery time for the whole set $B$, but due to the shift between $b_1$ and $b_2$ the average discovery time of $b_1$ neighbors is slightly higher compared to STEPOPT. The penalty for $b_1$ is compensated but the significant faster discovery of $b_3$ neighbors.

This example shows that the optimized listening schedule of a smaller beacon interval does not have to be a part of the optimized listening schedule of the next larger beacon interval in general regarding the minimization of the total average discovery time of beacon interval set $B$. Furthermore, the stepwise generation may also result in a propagation of error for each step of the computation.
Even though listening schedules that are computed stepwise for each beacon interval may not have minimal average discovery time, we use this idea in the design of our low-complexity algorithm \ALG{} which we will describe in Section~\ref{sec:alg_strategy}.

\begin{figure*}[ht]
\centering
    \subfloat[GENOPT]{
        \includegraphics[scale=0.8]{GENOPT_intervalSequence.jpg}
    }
    \subfloat[MINDY]{
        \includegraphics[scale=0.8]{ALG_intervalSequence.jpg}
    }
\caption{Listening schedules of the GENOPT and \ALG{} strategy for $|C| = 3$ and $B = \{1,2,3\}$.}
 \label{fig:intervalSequence}
\end{figure*}

\begin{table}
\centering
\caption{Analytical results of the average discovery time in time slots for each beacon interval $b$ as well as the beacon interval set $B =\{1,2,3\}$ and $|C| = 3$ }
\label{tab:intervalSequence}
\begin{tabular}{lrr}
  \hline  
                & GENOPT	&	\ALG{} \\  \hline
 $b_1$   			& 1.833		&	1.500 \\
 $b_2$   			& 3.000		&	3.000 \\
 $b_3$  			& 4.500		& 6.500 \\
 $B =\{1,2,3\}$	& 3.111		& 3.667 \\
  \hline
\end{tabular}
\end{table}


\subsection{\ALG{} strategy}

The STEPOPT and GENOPT strategies utilize linear optimization to obtain listening strategies. The decision variables are binary which results in a 0,1 / binary integer linear programming problem that are generally known to be NP hard.

Therefore a low-complex algorithm to compute listening schedules is desirable. In this section we present such an algorithm called \ALG{} which assembles the listening schedule stepwise for each beacon interval $b \in B$ starting with the smallest. Allocations of scans for the beacon interval $b_k$ which is currently being processed are stored in the variable $x_{c,t}$:

\[
x_{c,t} = \begin{cases}
              1 \textrm{, if a scan is performed on channel } c \textrm{ at time slot } t\\
              0 \textrm{, otherwise} %if no discovery is performed on channel } c \textrm{ at time slot } t
        \end{cases}
\]

When the processing of one beacon interval $b_k \in B$ is finished, the generated scheduled is stored in the variable $s_{c,t}$ which will be used as an input parameter for the computation of the schedule for the next larger beacon interval $b_{k+1}$. Before describing the algorithm in detail the term \textit{unique time slots} is introduced. For a beacon interval $b \in B$ and channel $c \in C$ a set of slot indices $U_{b,c} = \{u_{0,c}, u_{1,c}, \ldots, u_{b-1,c}\}$ is defined. Set $U_{b,c}$ describes the completeness of a scan for beacon interval $b$ on channel $c$. The entries $u_{i,c} \in U_{b,c}$ for $b \in B$ are defined as follows:

\begin{equation}
\begin{aligned} 
u_{i,c} = \begin{cases}
              1 \textrm{, if } \exists t \in T \textrm{ with } (x_{c,t} = 1 \vee s_{c,t} = 1) \wedge t \bmod b = i\\
              0 \textrm{, otherwise} 
        \end{cases}
\end{aligned}
\forall {c \in C} \;
\label{eq:ALG_unique_timeslots}
\end{equation}

If all entries $u_{i,c} \in U_{b,c}$ for a listening schedule are one, devices operating with beacon interval $b$ on any channel $c$ will be discovered when this schedule is performed under the assumptions stated in Section~\ref{sec:strategies}.

We will now explain the algorithm of \ALG{} to generate listening schedules. An overview of the algorithm is depicted in Figure~\ref{fig:alg_overview}. The algorithm consists of two steps in order to determine the allocation of the next scan $x_{c,t}$. In the first step the channel $c$ of the next allocation is selected and then the actual time slot $t$ in which the scan should take place is determined.

The algorithm starts with the smallest beacon interval $b_{min} = min(B)$. In the first step the unique time slots $u_{i,c}$ of the currently processed beacon interval $b_k$ are updated with the computed schedules $s_{c,t}$ of smaller BI. For $b_{min}$ all $u_{i,c}$ are zero. In the next step the elements of $U_{b_k,c}$ are analyzed for missing unique time slots (i.e. $u_{i,c} = 0$). 

If there are channels on which not all unique time slots are assigned yet, the average time per unique time slot is computed for all those channel $c \in C$.
For this purpose the first time slots $t$ on each channel $c$ for each $u_{i,c} \in U_{b_k,c}$ that are allocated in the current round $x_{c,t} = 1$ or have been allocated previously $s_{c,t} = 1$ with $(t \bmod b = i)$ are summed up. 
$(t + 0.5)$ is used when calculating the sum due to the assumption that in average a discovery will take place in the middle of a time slot.
Then the sum of each channel $c$ is divided by the number of $u_{i,c}$ with value one.
The channel with the lowest average time per unique time slot is selected, if two channels have identical values, priority is granted to the channel with the smaller number of unique time slots. The idea behind the selection is that new assignments of time slots are spread among the channels. Assigning an additional time slot to the channel with the lowest average time will result in an increased average time per unique time slot and therefore the channel will be less likely selected again in the next iteration.

After the selection of the channel the time slot on which the next scan should be performed has to be identified. 
For each missing unique time slot (i.e. $u_{i,c} = 0$) the next available time slot $t$ for a scan allocation on channel $c$ is computed, i.e. there are no scans scheduled $x_{c_1,t} = 0$ and $s_{c_1,t} = 0$ for all others channels $c_1 \neq c$. Among those possible time slots the largest time slot is selected and the scan $x_{c,t}$ added to the listening schedule for beacon interval $b_k$. \nie{[Tests with different beacon interval sets have shown that the selection of the largest time slot instead of the smallest resulted in significant reduction in the number of channel switchings of the generated listening schedules.]}

If all unique time slots $u_{i,c}$ of $b_k$ for all $c \in C$ are covered by scans $x_{c,t}$ for the beacon interval that is currently being processed or by scheduled scan $s_{c,t}$ for smaller beacon intervals, the listening schedule for $b_k$ is complete. If $b_k$ is the largest beacon interval of set $B$, the algorithm terminates and the computation of the listening schedule to discover neighbors operating with a beacon interval $b \in B$ on one channel $c \in C$ is finished. Otherwise, the whole computation starts again with the next larger beacon interval $b_{k+1}$.


\begin{figure}
\centering
\includegraphics{ALG_alg.jpg}
\caption{Computation of listening schedules of the low-complex discovery strategy \ALG{}}
\label{fig:alg_overview}
\end{figure}

\end{comment}
